When Less is More: Emerging Network-Wide Use Cases for Hollow-Core Fibers in Optical Networks [Invited]

Hollow-Core Fiber (HCF) is emerging as a disruptive technology for next-generation optical networks, offering 30\% lower propagation latency than standard Single-Mode Fiber (SMF), record-low attenuation (0.05-0.1 dB/km), and nonlinearities reduced by three to four orders of magnitude. While the physical-layer benefits of HCF have been extensively demonstrated, recent industrial commitments by hyperscalers (e.g., Microsoft, Amazon) and the rapid maturation of nested antiresonant nodeless fibers (NANF) call for a systematic assessment of the impact of HCF at the network level. Building on a series of prior contributions, we overview four emerging network-wide use cases for the selective deployment of HCF in hybrid SMF/HCF networks: (i) latency-constrained Edge Data Center (edgeDC) consolidation; (ii) energy-efficient high-power amplification; (iii) capacity scaling via single-fiber bidirectional (BiDi) transmission; and (iv) coexistence of classical and quantum (QKD) channels. Consolidated results across realistic metro, national, and continental topologies convey a unifying message: in each use case, a selective HCF upgrade captures a significant share of the achievable benefit compared to a network overhaul. The required HCF budget is use-case-specific, i.e., 6-24\% of the total network fiber length for edgeDC consolidation (up to 50\% fewer edgeDCs), 40\% of the network links for QKD/classical coexistence (up to 38\% fewer quantum modules), and 40-60\% of the network links for energy-efficient capacity scaling via BiDi-HCF (up to 28\% lower network power per Tbps and 70\% more served traffic, at half the HCF strand count of a unidirectional HCF upgrade), whereas for energy-efficient high-power amplification the gain keeps growing with the HCF budget (up to 60\% lower network power per Tbps at the national scale) and what saturates is the benefit of increasing the EDFA output power.

==> Figures/IT_ZRplus_percentage_vs_pout <==
% IT_ZRplus_percentage_vs_pout.tex
% Single subplot (single column): percentage of type-5 TXPs (ZR+) for IT topology
% for alpha/beta = 0.9/0.1 versus P_max.
% Budget % written above bars (rotated 90deg). Bars colored (same hue, increasing intensity).
% SSMF baseline shown as a black horizontal line (NO TEXT).

\begin{figure}[t]
\centering

% ===================== PARAMETERS =====================
\newcommand{\ZRymin}{0}
\newcommand{\ZRymax}{65}

\newcommand{\BarW}{8pt}                 % bar width
\newcommand{\BarGap}{0pt}               % gap between bars within a group

\newcommand{\BudgetLabelYShift}{-3pt}
\newcommand{\BudgetLabelXShift}{7pt}
% ======================================================

% --- derived bar spacing (keeps groups centered and prevents overlap) ---
\pgfmathsetlengthmacro{\BarStep}{\BarW+\BarGap}
\pgfmathsetlengthmacro{\ShiftA}{-1.5*\BarStep} % 25%
\pgfmathsetlengthmacro{\ShiftB}{-0.5*\BarStep} % 50%
\pgfmathsetlengthmacro{\ShiftC}{ 0.5*\BarStep} % 75%
\pgfmathsetlengthmacro{\ShiftD}{ 1.5*\BarStep} % 100%
% ---------------------------------------------------------

\pgfplotsset{
  ZRplusPctBarPlot/.style={
    ybar,
    bar width=\BarW,
    grid=both,
    major grid style={draw=gray!20},
    minor grid style={draw=gray!10},
    minor tick num=0,
    xminorgrids=false,
    tick align=outside,
    tick label style={font=\scriptsize},
    label style={font=\scriptsize},
    title style={font=\small},
    xtick={23,26,29,32,35},
    xmin=21.0, xmax=37.0,
    ymin=\ZRymin,
    ymax=\ZRymax,
    enlarge y limits={upper,value=0.06},
  }
}

% --- String row filter: keep only rows where column == value ---
\pgfplotsset{
  discard if not/.style 2 args={
    x filter/.code={
      \edef\cell{\thisrow{#1}}%
      \edef\want{#2}%
      \ifnum\pdfstrcmp{\cell}{\want}=0\relax
      \else
        \def\pgfmathresult{nan}%
      \fi
    }
  }
}

% Bars: lighter fills for better contrast with black text
\pgfplotsset{
  budget25/.style ={draw=blue!70!black, fill=blue!15},
  budget50/.style ={draw=blue!70!black, fill=blue!25},
  budget75/.style ={draw=blue!70!black, fill=blue!35},
  budget100/.style={draw=blue!70!black, fill=blue!45},
}

% Budget text above bars (rotated), black
\pgfplotsset{
  budgetText/.style={
    visualization depends on={value \thisrow{hcf_budget} \as \budgetlbl},
    nodes near coords={\budgetlbl\%},
    nodes near coords style={
      font=\scriptsize,
      rotate=90,
      anchor=south,
      inner sep=1pt,
      text=black
    },
    every node near coord/.append style={yshift=\BudgetLabelYShift, xshift=\BudgetLabelXShift},
  }
}

\begin{tikzpicture}

% Baseline (SSMF) percentage from first row in IT table
\pgfplotstableread[col sep=comma]{data/IT_raw/aggregated_IT.csv}\ITtable
\pgfplotstablegetelem{0}{mean_N_TXP_type5}\of\ITtable
\let\ITbaseTypeFive\pgfplotsretval
\pgfplotstablegetelem{0}{mean_N_TXP_total}\of\ITtable
\let\ITbaseTotalTxp\pgfplotsretval
\pgfmathsetmacro{\ITbaselineZRplusPct}{100*(\ITbaseTypeFive)/(\ITbaseTotalTxp)}

\begin{axis}[
  width=\columnwidth,
  height=0.45\columnwidth,
  ZRplusPctBarPlot,
  ylabel={ZR+ share (\%)},
  xlabel={$P_{\max}$ (dBm)},
]

% 25%
\addplot+[
  budget25, budgetText,
  bar shift=\ShiftA
] table[
    x=pout_max,
    y expr=100*(\thisrow{mean_N_TXP_type5})/(\thisrow{mean_N_TXP_total}),
    col sep=comma,
    discard if not={scenario}{HCF},
    restrict expr to domain={\thisrow{alpha}}{0.9:0.9},
    restrict expr to domain={\thisrow{beta}}{0.1:0.1},
    restrict expr to domain={\thisrow{hcf_budget}}{25:25},
    restrict expr to domain={\thisrow{pout_max}}{23.0:35.0},
  ] {data/IT_raw/aggregated_IT.csv};

% 50%
\addplot+[
  budget50, budgetText,
  bar shift=\ShiftB
] table[
    x=pout_max,
    y expr=100*(\thisrow{mean_N_TXP_type5})/(\thisrow{mean_N_TXP_total}),
    col sep=comma,
    discard if not={scenario}{HCF},
    restrict expr to domain={\thisrow{alpha}}{0.9:0.9},
    restrict expr to domain={\thisrow{beta}}{0.1:0.1},
    restrict expr to domain={\thisrow{hcf_budget}}{50:50},
    restrict expr to domain={\thisrow{pout_max}}{23.0:35.0},
  ] {data/IT_raw/aggregated_IT.csv};

% 75%
\addplot+[
  budget75, budgetText,
  bar shift=\ShiftC
] table[
    x=pout_max,
    y expr=100*(\thisrow{mean_N_TXP_type5})/(\thisrow{mean_N_TXP_total}),
    col sep=comma,
    discard if not={scenario}{HCF},
    restrict expr to domain={\thisrow{alpha}}{0.9:0.9},
    restrict expr to domain={\thisrow{beta}}{0.1:0.1},
    restrict expr to domain={\thisrow{hcf_budget}}{75:75},
    restrict expr to domain={\thisrow{pout_max}}{23.0:35.0},
  ] {data/IT_raw/aggregated_IT.csv};

% 100%
\addplot+[
  budget100, budgetText,
  bar shift=\ShiftD
] table[
    x=pout_max,
    y expr=100*(\thisrow{mean_N_TXP_type5})/(\thisrow{mean_N_TXP_total}),
    col sep=comma,
    discard if not={scenario}{HCF},
    restrict expr to domain={\thisrow{alpha}}{0.9:0.9},
    restrict expr to domain={\thisrow{beta}}{0.1:0.1},
    restrict expr to domain={\thisrow{hcf_budget}}{100:100},
    restrict expr to domain={\thisrow{pout_max}}{23.0:35.0},
  ] {data/IT_raw/aggregated_IT.csv};

% Baseline line (NO TEXT)
\addplot+[black, line width=1.2pt, no marks, sharp plot] coordinates {(21,\ITbaselineZRplusPct) (37,\ITbaselineZRplusPct)};

\end{axis}

\end{tikzpicture}

\caption{IT topology: percentage of type-5 transponders (ZR+) for $\alpha/\beta=0.9/0.1$ as a function of $P_{\max}$. Bars show HCF budgets (written above each bar); the horizontal line indicates the SSMF baseline.}
\label{fig:IT_ZRplus_percentage_vs_pout}
\end{figure}


==> Figures/IT_ZRplus_percentage_vs_pout_eb <==
% IT_ZRplus_percentage_vs_pout.tex
% Single subplot (single column): percentage of type-5 TXPs (ZR+) for IT topology
% for alpha/beta = 0.9/0.1 versus P_max.
% Budget % written above bars (rotated 90deg). Bars colored (same hue, increasing intensity).
% SSMF baseline shown as a black horizontal line (NO TEXT).

\begin{figure}[t]
\centering

% ===================== PARAMETERS =====================
\newcommand{\ZRymin}{0}
\newcommand{\ZRymax}{80}

\newcommand{\BarW}{8pt}                 % bar width
\newcommand{\BarGap}{0pt}               % gap between bars within a group

\newcommand{\BudgetLabelYShift}{-3pt}
\newcommand{\BudgetLabelXShift}{12pt}
% ======================================================

% --- derived bar spacing (keeps groups centered and prevents overlap) ---
\pgfmathsetlengthmacro{\BarStep}{\BarW+\BarGap}
\pgfmathsetlengthmacro{\ShiftA}{-1.5*\BarStep} % 25%
\pgfmathsetlengthmacro{\ShiftB}{-0.5*\BarStep} % 50%
\pgfmathsetlengthmacro{\ShiftC}{ 0.5*\BarStep} % 75%
\pgfmathsetlengthmacro{\ShiftD}{ 1.5*\BarStep} % 100%
% ---------------------------------------------------------

\pgfplotsset{
  ZRplusPctBarPlot/.style={
    ybar,
    bar width=\BarW,
    grid=both,
    major grid style={draw=gray!20},
    minor grid style={draw=gray!10},
    minor tick num=0,
    xminorgrids=false,
    tick align=outside,
    tick label style={font=\scriptsize},
    label style={font=\scriptsize},
    title style={font=\small},
    xtick={23,26,29,32,35},
    xmin=21.0, xmax=37.0,
    ymin=\ZRymin,
    ymax=\ZRymax,
    enlarge y limits={upper,value=0.06},
  }
}

% --- String row filter: keep only rows where column == value ---
\pgfplotsset{
  discard if not/.style 2 args={
    x filter/.code={
      \edef\cell{\thisrow{#1}}%
      \edef\want{#2}%
      \ifnum\pdfstrcmp{\cell}{\want}=0\relax
      \else
        \def\pgfmathresult{nan}%
      \fi
    }
  }
}

% Bars: lighter fills for better contrast with black text
\pgfplotsset{
  budget25/.style ={draw=blue!70!black, fill=blue!15},
  budget50/.style ={draw=blue!70!black, fill=blue!25},
  budget75/.style ={draw=blue!70!black, fill=blue!35},
  budget100/.style={draw=blue!70!black, fill=blue!45},
}

% Budget text above bars (rotated), black
\pgfplotsset{
  budgetText/.style={
    visualization depends on={value \thisrow{hcf_budget} \as \budgetlbl},
    nodes near coords={\budgetlbl\%},
    nodes near coords style={
      font=\scriptsize,
      rotate=90,
      anchor=south,
      inner sep=1pt,
      text=black
    },
    every node near coord/.append style={yshift=\BudgetLabelYShift, xshift=\BudgetLabelXShift},
  }
}

\begin{tikzpicture}

% Baseline (SSMF) percentage from first row in IT table
\pgfplotstableread[col sep=comma]{data/IT_raw/aggregated_IT.csv}\ITtable
\pgfplotstablegetelem{0}{mean_N_TXP_type5}\of\ITtable
\let\ITbaseTypeFive\pgfplotsretval
\pgfplotstablegetelem{0}{mean_N_TXP_total}\of\ITtable
\let\ITbaseTotalTxp\pgfplotsretval
\pgfmathsetmacro{\ITbaselineZRplusPct}{100*(\ITbaseTypeFive)/(\ITbaseTotalTxp)}

\begin{axis}[
  width=\columnwidth,
  height=0.45\columnwidth,
  ZRplusPctBarPlot,
  ylabel={ZR+ share (\%)},
  xlabel={$P_{\max}$ (dBm)},
]

% 25%
\addplot+[
  budget25, budgetText,
  error bars/y dir=both,
  error bars/y explicit,
  error bars/error bar style={black},
  error bars/error mark options={black, line width=0.4pt},
  bar shift=\ShiftA
] table[
    x=pout_max,
    y expr=100*(\thisrow{mean_N_TXP_type5})/(\thisrow{mean_N_TXP_total}),
    y error expr=100*sqrt((\thisrow{std_N_TXP_type5}/(\thisrow{mean_N_TXP_total}))^2 + ((\thisrow{mean_N_TXP_type5}*\thisrow{std_N_TXP_total})/(\thisrow{mean_N_TXP_total}^2))^2),
    col sep=comma,
    discard if not={scenario}{HCF},
    restrict expr to domain={\thisrow{alpha}}{0.9:0.9},
    restrict expr to domain={\thisrow{beta}}{0.1:0.1},
    restrict expr to domain={\thisrow{hcf_budget}}{25:25},
    restrict expr to domain={\thisrow{pout_max}}{23.0:35.0},
  ] {data/IT_raw/aggregated_IT.csv};

% 50%
\addplot+[
  budget50, budgetText,
  error bars/y dir=both,
  error bars/y explicit,
  error bars/error bar style={black},
  error bars/error mark options={black, line width=0.4pt},
  bar shift=\ShiftB
] table[
    x=pout_max,
    y expr=100*(\thisrow{mean_N_TXP_type5})/(\thisrow{mean_N_TXP_total}),
    y error expr=100*sqrt((\thisrow{std_N_TXP_type5}/(\thisrow{mean_N_TXP_total}))^2 + ((\thisrow{mean_N_TXP_type5}*\thisrow{std_N_TXP_total})/(\thisrow{mean_N_TXP_total}^2))^2),
    col sep=comma,
    discard if not={scenario}{HCF},
    restrict expr to domain={\thisrow{alpha}}{0.9:0.9},
    restrict expr to domain={\thisrow{beta}}{0.1:0.1},
    restrict expr to domain={\thisrow{hcf_budget}}{50:50},
    restrict expr to domain={\thisrow{pout_max}}{23.0:35.0},
  ] {data/IT_raw/aggregated_IT.csv};

% 75%
\addplot+[
  budget75, budgetText,
  error bars/y dir=both,
  error bars/y explicit,
  error bars/error bar style={black},
  error bars/error mark options={black, line width=0.4pt},
  bar shift=\ShiftC
] table[
    x=pout_max,
    y expr=100*(\thisrow{mean_N_TXP_type5})/(\thisrow{mean_N_TXP_total}),
    y error expr=100*sqrt((\thisrow{std_N_TXP_type5}/(\thisrow{mean_N_TXP_total}))^2 + ((\thisrow{mean_N_TXP_type5}*\thisrow{std_N_TXP_total})/(\thisrow{mean_N_TXP_total}^2))^2),
    col sep=comma,
    discard if not={scenario}{HCF},
    restrict expr to domain={\thisrow{alpha}}{0.9:0.9},
    restrict expr to domain={\thisrow{beta}}{0.1:0.1},
    restrict expr to domain={\thisrow{hcf_budget}}{75:75},
    restrict expr to domain={\thisrow{pout_max}}{23.0:35.0},
  ] {data/IT_raw/aggregated_IT.csv};

% 100%
\addplot+[
  budget100, budgetText,
  error bars/y dir=both,
  error bars/y explicit,
  error bars/error bar style={black},
  error bars/error mark options={black, line width=0.4pt},
  bar shift=\ShiftD
] table[
    x=pout_max,
    y expr=100*(\thisrow{mean_N_TXP_type5})/(\thisrow{mean_N_TXP_total}),
    y error expr=100*sqrt((\thisrow{std_N_TXP_type5}/(\thisrow{mean_N_TXP_total}))^2 + ((\thisrow{mean_N_TXP_type5}*\thisrow{std_N_TXP_total})/(\thisrow{mean_N_TXP_total}^2))^2),
    col sep=comma,
    discard if not={scenario}{HCF},
    restrict expr to domain={\thisrow{alpha}}{0.9:0.9},
    restrict expr to domain={\thisrow{beta}}{0.1:0.1},
    restrict expr to domain={\thisrow{hcf_budget}}{100:100},
    restrict expr to domain={\thisrow{pout_max}}{23.0:35.0},
  ] {data/IT_raw/aggregated_IT.csv};

% Baseline line (NO TEXT)
\addplot+[black, line width=1.2pt, no marks, sharp plot] coordinates {(21,\ITbaselineZRplusPct) (37,\ITbaselineZRplusPct)};

\end{axis}

\end{tikzpicture}

\caption{Percentage of ZR+ in case of IT for $\alpha/\beta=0.9/0.1$ as a function of $P_{\max}$. Bars show HCF budgets; the horizontal line indicates the SSMF baseline.}
\label{fig:IT_ZRplus_percentage_vs_pout_eb}
\end{figure}

